Exact Polynomial Time Algorithm for the Response Time Analysis of Harmonic Tasks with Constrained Release Jitter

In some important application areas of hard real-time systems, preemptive sporadic tasks with harmonic periods and constraint deadlines running upon a uni-processor platform play an important role. We propose a new algorithm for determining the exact worst-case response time for a task that has a lower computational complexity (linear in the number of tasks) than the known algorithm developed for the same system class. We also allow the task executions to start delayed due to release jitter if they are within certain value ranges. For checking if these constraints are met we define a constraint programming problem that has a special structure and can be solved with heuristic components in a time that is linear in the task number. If the check determines the admissibility of the jitter values, the linear time algorithm can be used to determine the worst-case response time also for jitter-aware systems.

==> proof.tex <==
 /* to be introduced in the Task Model section: */

The Processor Demand function $W_n(t)$ could be defined as follows:  

\begeq \label{eq:W}
W_n(t) \equals C_n + I_{n-1}(t) = C_n + \sig {i=1}{n-1} \cefr{t} {T_i}C_i
\endeq

We then define its least fixed point $R_n$ as: 

\begeq \label{eq:R}
R_n \equals \min \lef t| W(t) =t\ri
\endeq

\ssec {A different model for the total interference}
\sssec {Preliminary results of the exclusion intervals} \label{ssec:exclusionIntervals}
/* some introduction about the exclusion intervals of $R_n$ */

We now can formally demonstrate this property of exclusion intervals for $R_n$ as follows: 

\begle\label{le:exclusionIntervalR}
\begeq
\forall i = 1\dots n-1, \forall m_i \in N, R_n \notin (m_iT_i, m_iT_i + C_{i\dots n-1}] 
\endeq 
\endle
\begpro Supposing that $\exists i \in [1,n-1], m_i \in N$ such that $ m_iT_i < R_n \leq m_iT_i + C_{i\dots n-1} $, we will prove this lemma by counterposition.

By definition of \req {eq:R}, since $W_n(t)$ is a non-decreasing function with $W_n(0)>0$, and $R_n$ is the first instant that $W_n(t)=t$, we should have for all $t<R_n$, $W_n(t)>t$, hence $W_n(m_iT_i)>m_iT_i$. \hfill (*)\\
Also, we have: 

\begarr
W_n(R_n)-W_n(m_iT_i) &=& \sig {j=1}{n-1} \left( \cefr{R_n}{T_j} - \cefr {m_iT_i}{T_j} \right)C_j \nonumber\\
&=&\sig {j=1}{i-1} \left( \cefr{R_n}{T_j} - \cefr {m_iT_i}{T_j} \right)C_j \nonumber\\
 && + \sig {j=i}{n-1} \left( \cefr{R_n}{T_j} - \cefr {m_iT_i}{T_j} \right)C_j \nonumber\\
&\geq& \sig {j=i}{n-1} \left( \cefr{R_n}{T_j} - \cefr {m_iT_i}{T_j} \right)C_j \label{eq:mT-R}
\endarr

By nature of our reordered harmonic systems,  for all $j=i\dots n-1$, we have $T_j|T_i$ hence $T_j|m_iT_i$ and $\cefr {m_iT_i}{T_j}=\frac {m_iT_i}{T_j} <\frac {R_n}{T_j}\leq\cefr {R_n}{T_j}$. Therefore $\forall j \in [i,n-1], \cefr {R_n}{T_j}-\cefr {m_iT_i}{T_j} \geq 1$. Replacing these into \req{eq:mT-R} we have: 

\begarrno
W_n(R_n)-W_n(m_iT_i) &\geq& \sig {j=i}{n-1} C_j \\
W_n(R_n) &\geq& W_n(m_iT_i) + \sig {j=i}{n-1} C_j \\
R_n=W_n(R_n) &>& m_iT_i + C_{i\dots n-1} \text { (by (*))}
\endarrno
which contradicts that $R_n \in (m_iT_i, m_iT_i + C_{i\dots n-1}] $. The lemma is proved. 
\endpro
\sssec{A novel model to compute the task response times} \label{ssec:anotherModel}
/* some introduction about the model of $\widehat{I}$ and $\widehat{R}$ */\\
With such a model $\widehat{I}_{n-1}(t)$ of the interference, we can now define another Processor Demand function $\widehat{W}_{n}(t)$ as: 
\begeq \label{Wh}
\widehat{W}_{n}(t)  \equals C_n+ \widehat{I}_{n-1}(t) = C_n + \sig {i=1}{n-1} \cefr{t-C_{i+1\dots n-1}} {T_i}C_i
\endeq 
We then obtain its least fixed point $\widehat{R}_{n}$ as: 
\begeq\label{Rh}
\widehat{R}_{n} \equals \min \lef t| \widehat{W}_{n}(t) =t\ri
\endeq

We will now demonstrate that this novel analysis model of  $\widehat{I}_{n-1}(t)$,  $\widehat{W}_{n}(t)$ and  $\widehat{R}_{n}$ is equivalent to the response time analysis of ${I}_{n-1}(t)$,  ${W}_{n}(t)$ and  ${R}_{n}$. For this purpose, we first present the following property of  $\widehat{R}_{n}$:

\begle\label{le:exclusionIntervalRh}
\begeq
\forall i = 1\dots n-1, \forall m_i \in N, \widehat{R}_{n} \notin (m_iT_i, m_iT_i + C_{i\dots n-1}] 
\endeq 
\endle
\begpro
Supposing that $\exists i \in [1,n-1], m_i \in N$ such that $ m_iT_i < \widehat{R}_n \leq m_iT_i + C_{i\dots n-1} $, we will prove this lemma by counterposition.

Note also that since $\widehat{W}_{n}(t)$ is a non-decreasing function with $\widehat{W}_{n}(0)>0$, and $\widehat{R}_n$ is the first instant that $\widehat{W}_{n}(t)=t$, we should have for all $t<\widehat{R}_n, \widehat{W}_{n}(t)>t$. \hfill (*)\\ 

Now we will prove that $\widehat{R}_n> m_iT_i+ C_{i..n-1}$ by induction. \\
1. First we prove the base case that $ \widehat{R}_n> m_iT_i+C_{n-1}$. 

Since by definition, $\widehat{W}_n(\widehat{R}_n) = \widehat{R}_n$, we have: 
\begarr
\widehat{R}_n-\widehat{W}_n(m_iT_i)&=&\widehat{W}_n(\widehat{R}_n)-\widehat{W}_n(m_iT_i) \nonumber\\
&=& \sig {j=1}{n-1} \left( \cefr{\widehat{R}_n-C_{j+1..n-1}}{T_j} - \cefr {m_iT_i- C_{j+1..n-1}}{T_j} \right)C_j \label{eq:base}
\endarr

Let us consider the addends of the accumulate sum above: 

- For $j =1..n-2$: Since $\widehat{R}_n > m_iT_i$ we have: 

\begeq \label{eq:jBeforeLast}
\drop{i=1..n-2,}\cefr{\widehat{R}_n-C_{j+1..n-1}}{T_j} - \cefr {m_iT_i- C_{j+1..n-1}}{T_j} \geq 0
 \endeq

- For $j=n-1$:  By nature of our reordered harmonic systems, with $i\leq n-1$, we have $T_{n-1}|T_i$ hence $T_{n-1}|m_iT_i$ and $\cefr {m_iT_i}{T_{n-1}}=\frac {m_iT_i}{T_{n-1}} <\frac {\widehat{R}_n}{T_{n-1}}\leq\cefr {\widehat{R}_n}{T_{n-1}}$. Therefore, with $j=n-1$:

 \begeq\label{eq:jLast}
\drop{j= n-1,} \cefr {\widehat{R}_n}{T_{j}}-\cefr {m_iT_i}{T_{j}} \geq 1
\endeq

Applying \req{eq:jBeforeLast} and \req{eq:jLast} into \req{eq:base}, we have $\widehat{R}_n - \widehat{W}_n(m_iT_i)\geq C_{n-1}$. By (*), we also have $\widehat{W}_n(m_iT_i)>m_iT_i$, hence $\widehat{R}_n \geq m_iT_i+ C_{n-1}$ and the base case is proved. \\
2. Now supposing we already had $\widehat{R}_n> m_iT_i+ C_{k..n-1}$ with $i+1\leq k\leq n-1$ we will prove that $\widehat{R}_n>  m_iT_i+ C_{k-1 ..n-1}$. We have:  

\begarr
&&\widehat{R}_n-\widehat{W}_n(m_iT_i+C_{k..n-1})=\widehat{W}_n(\widehat{R}_n)-\widehat{W}_n(m_iT_i+C_{k..n-1}) \nonumber\\
&&= \sig {j=1}{n-1} \left( \cefr{\widehat{R}_n-C_{j+1..n-1}}{T_j} - \cefr {m_iT_i +C_{k..n-1}- C_{j+1..n-1}}{T_j} \right)C_j \label{eq:inductive}
\endarr

Let us consider the addends of the accumulate sum above: 

- For $j =1.. n-1, j!=k-1$: Since by the inductive hypothesis $\widehat{R}_n >  m_iT_i+ C_{k..n-1}$, we have: 

\begeq \label{eq:jBeforeLastInductive}
 \drop{j =1.. n-1, j!=k-1,} \cefr{\widehat{R}_n-C_{j+1..n-1}}{T_j} - \cefr {m_iT_i+ C_{k..n-1}- C_{j+1..n-1}}{T_j} \geq 0
 \endeq

- For $j=k-1$: By the inductive hypothesis, we have $\widehat{R}_n-C_{j+1..n-1}>m_iT_i+ C_{k..n-1}- C_{j+1..n-1}= m_iT_i$. Also, $i+1\leq k \infer k-1 \geq i$, then by nature of our reordered harmonic systems, we have $T_{k-1}|T_i$ hence $T_{k-1}|m_iT_i$ and $\cefr {m_iT_i}{T_{k-1}} =\frac {m_iT_i}{T_{k-1}}$. Combine all these we have $\frac{\widehat{R}_n-C_{j+1..n-1}}{T_{j}} >\frac {m_iT_i}{T_{k-1}}=\cefr {m_iT_i}{T_{k-1}}= \cefr {m_iT_i+ C_{k..n-1}- C_{j+1..n-1}}{T_j}$. Finally, applying $\ceil{x}\geq x$, for $j=k-1$ we obtain:  

 \begeq\label{eq:jLastInductive}
\drop{j=k-1,} \cefr{\widehat{R}_n-C_{j+1..n-1}}{T_j} - \cefr {m_iT_i+ C_{k..n-1}- C_{j+1..n-1}}{T_j} \geq 1
\endeq

 Applying \req{eq:jBeforeLastInductive} and \req{eq:jLastInductive} into \req{eq:inductive}, we have $\widehat{R}_n -\widehat{W}_n(m_iT_i+ C_{k..n-1}) \geq  C_{k-1}$. Also, by (*), $\widehat{W}_n(m_iT_i+ C_{k..n-1})>m_iT_i+ C_{k..n-1}$. Consequently, we have $\widehat{R}_n > m_iT_i+ C_{k-1..n-1}$ and the inductive case is proved. 

Finally, applying the results above inductively from the base case until $k=i+1$, we have $\widehat{R}_n > m_iT_i+ C_{i..n-1}$, which contradicts the counterpositive hypothesis and the lemma is proved.  
\endpro

Now having this property of exclusion intervals for $\widehat{R}_{n}$, we could prove the correctness of the novel response time analysis: 

\begle\label{le:RRh}
\begeq
R_n = \widehat{R}_n
\endeq
\endle
\begpro  We compare the associated ceiling functions composing $W_n(t)$ and $\widehat{W}_n(t)$:

 $$\left\lceil t/T_j\right\rceil \\\ \text{and} \\\left\lceil t-C_{j+1\ldots n-1}/T_j\right\rceil$$

The two terms have the same value for $m_jT_j+C_{j+1\ldots n-1} {<} t {\leq}  (m_j+1)T_{j}$ for any $j \in[1, n-1]$.  \hfill (*)


By \rle{le:exclusionIntervalR}, the times of (*) are contained in the permissible value range of ${R}_n$. Therefore for $t = {R}_n$ we obtain $ W_n(t)=\widehat{W}_n(t)$. Since for $t = {R}_n, {W}_n(t) =t $ then for $t = {R}_n, \widehat{W}_n(t) =t$, i.e., ${R}_n$ is a fixed point of the equation $\widehat{W}_n(t)=t$. Also, by definition, $\widehat{R}_n$ is the least fixed point of $\widehat{W}_n(t)=t$, hence we have $\widehat{R}_n \leq R_n$.  \hfill(**)

 
Now by \rle{le:exclusionIntervalRh}, the times of (*) are also contained in the permissible value range of $\widehat{R}_n$. Therefore for $t = \widehat{R}_n$, we also obtain $W_n(t)=\widehat{W}_n(t)$. Since for $t = \widehat{R}_n, \widehat{W}_n(t) =t $ then for $t = \widehat{R}_n, W_n(t) = t$, i.e., $\widehat{R}_n$ is a fixed point of the equation $W_n(t) =t$. Since $R_n$ is the least fixed point of $W_n(t)=t$, we have $R_n\leq\widehat{R}_n$. \hfill(***)

From (**) and (***), the lemma is proved. 

\endpro
